A two-layer approach for Coupling 1D/2D Shallow Water Flow Models

In this paper, we propose a novel approach for coupling 2D/1D shallow water flow models. Efficiently coupling these models is vital for simulating the flow and flooding of open channels. Currently, existing methods couple the models either at the channel lateral boundaries (lateral methods) or at the location, along the channel flow direction, where the two sub-domains intersect (frontal methods). We classify these methods as horizontal methods since the coupling points are on the horizontal plane. The limitations of these methods include their inability to recover the 2D channel flow structure during flooding without losing efficiency, and their inability to switch between lateral and frontal methods, based on the problem. Here, we propose a new paradigm which is to think of the channel flow as a two layer flow. This leads to the vertical coupling method (VCM) which is able to recover 2D channel flow structure without losing efficiency, switch types depending on the flow and is a superset of some existing methods. The VCM is based on a user chosen elevation above which the user considers the channel to be full. From this elevation, all other flow quantities are defined including the two layers. The flows in the lower and upper layers are assumed to be 1D and 2D respectively, and the appropriate flow models with exchange terms are derived. The 2D shallow water flow model is retained for the floodplains. Finite volume methods (FVM) are formulated for the flood model; the FVM with the operator splitting approach are also formulated to solve and couple the two layer channel flow models. We show that the resulting method (i) is well-balanced (ii) preserves the "no-numerical" flooding property (iii) preserves conservation properties and (iv) adapts to the flow situation.

==> abstract.tex <==
% ABSTRACT
%
%
%
Efficient coupling methods for 2D/1D shallow water flow models are vital for simulating
the flow and flooding of open channels. Existing methods
couple the models either at the channel lateral boundaries (lateral methods)
or at the location, along the channel flow direction, where the two sub-domains intersect 
(frontal methods). We categorise these methods as horizontal methods since the coupling
points are on the horizontal plane. 
The limitations of these methods include their inability to recover the
true 2D channel flow structure during flooding without losing efficiency, and
their inability to switch between lateral and frontal methods, according to the situations.
In this paper, we propose a new paradigm which is to think of the channel flow as a 
two layer flow. This leads to the  vertical coupling method (VCM)  which
is able to recover 2D channel flow structure without losing efficiency, switch types
according to the flow situation and is a superset of some existing methods. 
The VCM is based on a user chosen elevation above which the user considers
the channel to be full. From this elevation, all other flow quantities are defined
including the two layers. The flows in the lower and upper layers
are assumed to be 1D and 2D respectively, and the appropriate flow models with 
exchange terms are derived. The 2D shallow water flow model
is retained for the floodplains.
Finite volume methods (FVM) are formulated for the flood model; the FVM
with the operator splitting approach are also formulated to solve and couple the two layer
channel flow models. 
We show that the resulting method (i) is well-balanced (ii) preserves the "no-numerical" flooding property
(iii) preserves conservation properties and
(iv) adapts to the flow situation.
Numerical results show that the method performs well in terms of accuracy,
and recovers the channel 2D flow structure whenever flooding.
%We also discuss (without numerical details) how the method is a family of methods.

==> concl.tex <==
The problem of coupling the 2D and 1D shallow water equations have been investigated in this paper.
We focused on the need to efficiently recover 2D channel flow structure during flood while maintaining
good accuracy. To this end, the vertical coupling method is proposed for the first time. 
We show that the method truly recovers the 2D flow structure, is a unifying method, mass conservative,
well-balanced and preserves the no-numerical flooding property. In addition, the numerical results
show that the VCM, in most cases, outperforms the existing methods compared with it in this
paper. 

==> scheme-intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%                               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  Introduction                 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%                               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we detail the numerical schemes for the models presented in previous sections.
%To begin, we partition the channel into a 1D grid, 
%$\Omega_h^{1D}$ made of cross sections and the floodplains, into a 2D grid $\Omega_h^{2D}$,
%see figure \ref{fig2d1dgrid}. We first present the scheme for the 2D flood model, then
%the schemes for the channel flow model is presented.
%
%
%\begin{figure}[ht!]
% \subfigure[Grid of the entire domain consisting of the 1D grid $\Omega_h^{1D}$ at the middle and the 2D grids $\Omega_h^{2D}$ for the floodplains.]
%          {\label{fig2d1dgrid}\includegraphics[width=0.5\textwidth, height=0.35\textwidth]{2d1dgrid}}
%\hspace{0.02\textwidth}
%%
% \subfigure[2D mesh showing two neighbour cells, $T_j$ and $T_k$, the edge $e_{jk}$ between them and the normal vector $\vec{n}_{jk}$.]
%          {\label{fvm-fig-single2dmesh}\includegraphics[width=0.4\textwidth, height=0.35\textwidth]{single2dmesh}}
%\end{figure}
Let $\{ x_{i+1/2}\}_{i=0}^{N_x^1}$ be set of points along the channel and
$ x_i = \left(  x_{i-1/2} + x_{i+1/2} \right)/2 $, then we partition the channel,  $\Omega_c$ (see figure \ref{horifigriverfloodplain})
into a $1D$ mesh, $\Omega_h^1$ made up of cells, $K_i = (x_{i-1/2}, x_{i+1/2} )$ (see figure \ref{vertnumfig1dmesh}).
We further discretize the channel into a 2D mesh $\Omega^2_h$ such that each 2D cell, $T_{ij}$ is a subcell of a unique 1D cell, $K_i \in \Omega_h^1$,
that is,
\begin{align}\label{vertnumeqncells}
	\Omega_h^2 = \{  T_{ij} :  \exists ! K_i \in \Omega_h^1 \mbox{ such that } T_{i,j} \in K_i   \},    %\bigcup_{j=1}^{N_y^1}T_{ij} 
\end{align}
see figure \ref{vertnumfig2dmesh}.
We also discretize time as, $t^n, n=1,2,...N^n$.

\begin{figure}[ht!]
  \begin{center}
  \subfigure[Top view of 1D channel mesh made of cells $K_i$. The lower layer model is to be solved on each cell, $K_i$.]
   {\label{vertnumfig1dmesh} \includegraphics[width=0.44\textwidth]{vcm-1dmesh}}
  \hspace*{0.03\textwidth}
   \subfigure[Top view of 2D mesh for the channel region only - no floodplains. Each 1D channel cell $K_i$ (in red)  
              is further discretized to form a number, $N_y^1$ of 2D cells, $T_{ij}, j=1,2,..., N_y^1$.]
              {\label{vertnumfig2dmesh} \includegraphics[width=0.48\textwidth]{vcm-mesh-2d-upper-layer}}   
  \end{center}
  \caption{Mesh for the two sub-models. }
\end{figure}
